Optimal Rates and Efficient Algorithms for Online Bayesian Persuasion

Bayesian persuasion studies how an informed sender should influence beliefs of rational receivers who take decisions through Bayesian updating of a common prior. We focus on the online Bayesian persuasion framework, in which the sender repeatedly faces one or more receivers with unknown and adversarially selected types. First, we show how to obtain a tight $\tilde O(T^{1/2})$ regret bound in the case in which the sender faces a single receiver and has partial feedback, improving over the best previously known bound of $\tilde O(T^{4/5})$. Then, we provide the first no-regret guarantees for the multi-receiver setting under partial feedback. Finally, we show how to design no-regret algorithms with polynomial per-iteration running time by exploiting type reporting, thereby circumventing known intractability results on online Bayesian persuasion. We provide efficient algorithms guaranteeing a $O(T^{1/2})$ regret upper bound both in the single- and multi-receiver scenario when type reporting is allowed.

==> defs.tex <==
\declaretheorem[name=Theorem]{thm}
\declaretheorem[name=Corollary]{cor}
\declaretheorem[name=Lemma]{lem}

\newcommand{\Bigtimes}{\text{\LARGE $\times$}}
\newcommand{\I}{\mathcal{I}}
\newcommand{\J}{\mathcal{J}}
\newcommand{\A}{\mathcal{A}}
\newcommand{\Si}{\mathcal{S}}
\newcommand{\Z}{\mathcal{Z}}
\newcommand{\N}{\mathcal{N}}
\newcommand{\C}{\mathcal{C}}
\newcommand{\B}{\mathcal{B}}
\newcommand{\Hi}{\mathcal{H}}
\newcommand{\Pical}{\mathcal{P}}
\newcommand{\thetavec}{\boldsymbol{\theta}}
\newcommand{\omegavec}{\boldsymbol{\omega}}
\newcommand{\pivec}{\boldsymbol{\pi}}
\newcommand{\xivec}{\boldsymbol{\xi}}
\newcommand{\defeq}{\coloneqq}
\newcommand{\Reals}{\mathbb{R}}
\newcommand{\nvec}{\boldsymbol{n}}
\newcommand{\xvec}{\boldsymbol{x}}
\newcommand{\rhovec}{\boldsymbol{\rho}}
\newcommand{\phivec}{\boldsymbol{\phi}}
\newcommand{\muvec}{\boldsymbol{\mu}}
\newcommand{\pvec}{\boldsymbol{p}}
\newcommand{\yvec}{\boldsymbol{y}}
\newcommand{\zvec}{\boldsymbol{z}}
\newcommand{\lambdavec}{\boldsymbol{\lambda}}
\newcommand{\nuvec}{\boldsymbol{\nu}}
\newcommand{\kvec}{\boldsymbol{k}}
\newcommand{\zerovec}{\boldsymbol{0}}
\newcommand{\Fmat}{\boldsymbol{F}}
\newcommand{\Rmat}{\boldsymbol{R}}
\newcommand{\Ovec}{\boldsymbol{O}}
\newcommand{\Nvec}{\boldsymbol{N}}
\newcommand{\fvec}{\boldsymbol{f}}
\newcommand{\Y}{\mathcal{Y}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\Umat}{\boldsymbol{U}}
\newcommand{\fict}{\overline{I}}
\newcommand{\bvec}{\boldsymbol{b}}
\newcommand{\cvec}{\boldsymbol{c}}
\newcommand{\Amat}{\boldsymbol{A}}
\newcommand{\vvec}{\boldsymbol{v}}
\newcommand{\Imat}{\boldsymbol{I}}
\newcommand{\inst}[1]{\mathfrak{#1}}
\newcommand{\argmax}{\operatornamewithlimits{argmax}}
\newcommand{\uvec}{\boldsymbol{u}}
\newcommand{\omvec}{\boldsymbol{\omega}}
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
		\node[shape=circle,draw,inner sep=0.9pt] (char) {#1};}}
	
	\newcommand{\pers}{\Phi^\diamond}
	
% underbar
\newcommand{\munderbar}[1]{\underaccent{\bar}{#1}}

% definitions particular
\newcommand{\us}{f} %sender utility terminal
\newcommand{\ur}{u} %receiver utility terminal
\newcommand{\U}{F} %sender utility
\newcommand{\V}{U} %receiver utility
\newcommand{\Rs}{R} % regret sender
\newcommand{\Rr}{V} % regret receiver
%\newcommand{\us}{\clubsuit} %sender utility terminal
%\newcommand{\ur}{\spadesuit} %receiver utility terminal
%\newcommand{\U}{\bigstar} %sender utility
%\newcommand{\V}{\blacksquare} %receiver utility
%\newcommand{\Rs}{\blacktriangle} % regret sender
%\newcommand{\Rr}{\blacklozenge} % regret receiver


\newtheorem{example}{Example}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{remark}{Remark}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{definition}{Definition}
\newtheorem{assumption}{Assumption}

%Theorems
\declaretheorem[name=Theorem,numberwithin=section]{thr}
\declaretheorem[name=Definition,numberwithin=section]{defi}
\declaretheorem[name=Proposition,numberwithin=section]{prop}
\declaretheorem[name=Assumption,numberwithin=section]{ass}
\declaretheorem[name=Corollary,numberwithin=section]{coroll}
\declaretheorem[name=Fact,numberwithin=section]{fact}



%=== COLORED COMMENTS =====================================================================================
\usepackage{pifont}
\usepackage[normalem]{ulem} % for \sout

\newcommand{\ugh}[1]{{\color{red}{\uwave{#1}}}} % please rephrase
\newcommand{\ins}[1]{{\color{blue}{\uline{#1}}}} % please insert
\newcommand{\del}[1]{{\color{red}{\sout{#1}}}} % please delete
\newcommand{\chg}[2]{\del{#1}\ins{#2}} % please change
\newcommand{\sugg}[1]{{\color{orange}{#1}}}
% \newcommand{\todo}[2][]{{\color{blue}{\textbf{[TODO #1]} #2}}}

\definecolor{mygreen}{rgb}{0.0, 0.5, 0.0}
\definecolor{myorange}{rgb}{0.55, 0.62, 1}
\newcommand{\nb}[3]{{\colorbox{#2}{\bfseries\sffamily\scriptsize\textcolor{white}{#1}}}{\textcolor{#2}{\sf\small\textsf{#3}}}}

\newcommand{\mat}[1]{\nb{Matteo}{purple}{#1}}
\newcommand{\alb}[1]{\nb{Albo}{blue}{#1}}
\newcommand{\ma}[1]{\nb{Marti}{myorange}{#1}}
\newcommand{\fe}[1]{\nb{Federico}{mygreen}{#1}}
\newcommand{\fr}[1]{\nb{Fra}{magenta}{#1}}
\newcommand{\nc}[1]{\nb{Nicola}{violet}{#1}}

\allowdisplaybreaks

%%% names
\newcommand{\LP}{\text{LP}}

==> pckgs.tex <==
\usepackage{amsfonts}
\usepackage{multicol}
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
\usepackage{mathtools}
\usepackage{amsthm}
\usepackage{thmtools}
\usepackage{thm-restate}
\usepackage{lipsum}
\usepackage{amssymb }
\usepackage{mleftright}
\usepackage{color}
\usepackage{diagbox}
\usepackage{tikz}
\usepackage{wrapfig}
\usetikzlibrary{positioning,fit,calc,matrix,arrows,trees,backgrounds}
\usepackage{accents}
\usepackage{tikz}
\usepackage{pgfplots}
\usepackage{enumerate}
\usepackage[shortlabels]{enumitem}
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{xcolor}         % colors



